Restore Anything Model via Efficient Degradation Adaptation

With the proliferation of mobile devices, the need for an efficient model to restore any degraded image has become increasingly significant and impactful. Traditional approaches typically involve training dedicated models for each specific degradation, resulting in inefficiency and redundancy. More recent solutions either introduce additional modules to learn visual prompts significantly increasing model size or incorporate cross-modal transfer from large language models trained on vast datasets, adding complexity to the system architecture. In contrast, our approach, termed RAM, takes a unified path that leverages inherent similarities across various degradations to enable both efficient and comprehensive restoration through a joint embedding mechanism without scaling up the model or relying on large multimodal models. Specifically, we examine the sub-latent space of each input, identifying key components and reweighting them in a gated manner. This intrinsic degradation awareness is further combined with contextualized attention in an X-shaped framework, enhancing local-global interactions. Extensive benchmarking in an all-in-one restoration setting confirms RAM's SOTA performance, reducing model complexity by approximately 82% in trainable parameters and 85% in FLOPs. Our code and models will be publicly available.

==> figs/model_complexity.tex <==
\begin{tikzpicture}[baseline]

\begin{axis}[
    width=\textwidth,
    height=0.65\textwidth,
    xtick pos=left,
    ytick pos=left,
    xlabel near ticks,
    ylabel near ticks, 
    ymin = 25,
    ymax = 33,
    xmin = 0,
    xmax = 50,
    xlabel={Parameters (M)},
    ylabel={PSNR (dB)},
    grid,
    grid style=dashed,
   % title={Avg. PSNR},
    title style={anchor=north, at={(0.5,1.1)},},
    tick label style={font=\scriptsize}, % Set the font size for tick labels
    title style={font=\scriptsize}, % Set the font size for the title
    label style={font=\scriptsize}, % Set the font size for the axis 
    nodes near coords, % Add text label
    enlarge y limits=0.1,
    enlarge x limits=0.1,
    legend style={at={(.2,.925)}, anchor=center, legend columns=-1, font=\tiny,},
    ]
    
    \addplot[
    nodes near coords style = {font=\scriptsize, anchor=south west, xshift=-2pt},
    scatter/classes={
            b={color=tabblue!50, mark size=1.7},
            c={color=taborange!50, mark size=1.7}
            },
    scatter, mark=*, only marks, 
    scatter src=explicit symbolic,
    nodes near coords*={\Label},
    visualization depends on={value \thisrow{label} \as \Label} 
    ] table [meta=class] {
    x y class label
    %2 29.98 b DL
    16 30.17 b MPRNet
    9 31.20 b AirNet
    36 32.06 b PromptIR
    %16 32.33 b DyNet-L
    %29 32.69 b AdaIR
    15 28.34 c IDR
    9 25.49 c AirNet
    1 25.09 c TAPE
    };

    \addplot[
    nodes near coords style = {font=\scriptsize, anchor=south west, xshift=-2pt, color=tabblue},
    scatter/classes={
            a={color=tabblue, mark size=1.7},
            d={color=taborange, mark size=1.7}
            },
    scatter, mark=*, only marks, scatter src=explicit symbolic, nodes near coords*={\Label},
    visualization depends on={value \thisrow{label} \as \Label} 
    ] table [meta=class] {
    x y class label
    6 32.51 a Ours 
    };

    \addplot[
    nodes near coords style = {font=\scriptsize, anchor=north west, xshift=-1pt, color=taborange},
    scatter/classes={
            d={color=taborange, mark size=1.7}
            },
    scatter, mark=*, only marks, scatter src=explicit symbolic, nodes near coords*={\Label},
    visualization depends on={value \thisrow{label} \as \Label} 
    ] table [meta=class] {
    x y class label
    6 30.24 d Ours
    };

    % comparison to IDR
    \draw[gray, line width=0.75pt] (axis cs:15, 28.34) -- (axis cs:6, 28.34);
    \draw[-stealth, gray, line width=0.75pt] (axis cs:6, 28.34) -- (axis cs:6, 30.04);
    \node at (axis cs:10, 28) {\tiny\textcolor{red}{-$60\%$}};
    \node at (axis cs:1, 29) {\tiny\textcolor{red}{+$1.9$dB}};
    
    % comparison to AirNet
    \draw[gray, line width=0.75pt] (axis cs:9, 31.20) -- (axis cs:6, 31.20);
    \draw[-stealth, gray, line width=0.75pt] (axis cs:6, 31.20) -- (axis cs:6, 32.25);
    \node at (axis cs:4, 30.95) {\tiny\textcolor{red}{-$33\%$}};
    \node at (axis cs:1, 32) {\tiny\textcolor{red}{+$1.2$dB}};
    
    % add legend
    \draw[draw=tabblue, fill=tabblue] (340, 100) circle [radius=0.05cm];
    \node[text width=1.5cm] at (435,100) {\tiny 3 Degredations};
    \draw[draw=taborange, fill=taborange] (340, 10) circle [radius=0.05cm];
    \node[text width=1.5cm] at (435, 10) {\tiny 5 Degredations};
\end{axis}
\end{tikzpicture}

==> tables/ab_data.tex <==
\begin{table}[!t]
    \centering
    \footnotesize
    %\setlength\tabcolsep{1pt}
    %\setlength{\extrarowheight}{0.5pt}
    \caption{\textbf{Average} results for \textit{denoising} and \textit{overall} (\ie, dehazing, draining, and denoising) under the 3-degradation IR setting.}
    \label{tab:ab_data}
    \vspace{-2mm}
    \begin{tabularx}{\columnwidth}{X*{5}{c}}
        \toprule
         Method & \multicolumn{2}{c}{Denoising} & \multicolumn{2}{c}{Overall} \\ 
         %\cline{2-3} \cline{4-5} 
         %& PSNR(dB, $\uparrow$) & SSIM ($\uparrow$) & PSNR(dB, $\uparrow$) & SSIM ($\uparrow$)\\ 
         \midrule
        PromptIR~\cite{potlapalli2023promptir} & 31.11 & \cellcolor{clblue!50}.873 & 32.06 & \cellcolor{clblue!50}.913 \\ \midrule
        \ourmethod (Original,ours) & 31.09 & \cellcolor{clblue!50}.873 & 32.51 & \cellcolor{clblue!50}.916 \\
        \ourmethod (New, ours) & \textbf{31.24} & \cellcolor{clblue!50}\textbf{.877} & \textbf{32.58} & \cellcolor{clblue!50}\textbf{.919} \\  
        \bottomrule        
    \end{tabularx}
    \vspace{-5mm}
\end{table}

==> tables/supp_3deg.tex <==
\begin{table*}[t]
    \centering
    \footnotesize
    \fboxsep0.75pt
    %\setlength\tabcolsep{2pt}
    \setlength{\extrarowheight}{0.8pt}
    \caption{\textit{Comparison to state-of-the-art on three degradations.} PSNR (dB, $\uparrow$) and SSIM ($\uparrow$) metrics are reported on the full RGB images. \textcolor{tabred}{\textbf{Best}} and \textcolor{tabblue}{\textbf{second best}} performances are highlighted. Our method sets a new state-of-the-art on average across all benchmarks while being significantly more efficient than prior work. ‘-’ represents unreported results.}
    \vspace{-3mm}
    \label{tab:exp:supp_3deg}
    \begin{tabularx}{\textwidth}{X*{16}{c}}
    \toprule
     \multirow{2}{*}{Method} & \multirow{2}{*}{Num.Blocks} &\multirow{2}{*}{Params.} 
     & \multicolumn{2}{c}{\textit{Dehazing}} & \multicolumn{2}{c}{\textit{Deraining}} & \multicolumn{6}{c}{\textit{Denoising}} 
     & \multicolumn{2}{c}{\multirow{2}{*}{Average}}  \\
     \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-13} 
     & & & \multicolumn{2}{c}{SOTS} & \multicolumn{2}{c}{Rain100L} & \multicolumn{2}{c}{BSD68\textsubscript{$\sigma$=15}} & \multicolumn{2}{c}{BSD68\textsubscript{$\sigma$=25}} & \multicolumn{2}{c}{BSD68\textsubscript{$\sigma$=50}} &  \\
     \midrule
     \rowcolor{gray!10} Base~\cite{potlapalli2023promptir} & [4,6,6,8] &36M & \textcolor{tabblue}{\textbf{30.58}} & \textcolor{tabblue}{\textbf{.974}} & \textcolor{tabblue}{\textbf{36.37}} &  \textcolor{tabblue}{\textbf{.972}} & \textcolor{tabred}{\textbf{33.98}} &  \textcolor{tabred}{\textbf{.933}} & \textcolor{tabred}{\textbf{31.31}} & \textcolor{tabblue}{\textbf{.888}} & \textcolor{tabred}{\textbf{28.06}} &  \textcolor{tabred}{\textbf{.799}} & \textcolor{tabblue}{\textbf{32.06}} &  \textcolor{tabblue}{\textbf{.913}} \\
     Base~\cite{potlapalli2023promptir} & [3,5,5,7] & 32M & 30.70 & .978 & 37.39 & .977 & 33.05 & .909 & 30.65 & .863 & 27.96 & .793 & 31.95 & .904\\
     \ourmethod (\textit{Ours}) & [3,5,5,7] &\textcolor{tabred}{\textbf{6M}} & \textcolor{tabred}{\textbf{31.38}} &  \textcolor{tabred}{\textbf{.979}} & \textcolor{tabred}{\textbf{37.90}} &  \textcolor{tabred}{\textbf{.981}} & \textcolor{tabblue}{\textbf{33.95}} &  \textcolor{tabred}{\textbf{.933}} & \textcolor{tabblue}{\textbf{31.30}} & \textcolor{tabred}{\textbf{.889}} & \textcolor{tabblue}{\textbf{28.04}} & \textcolor{tabblue}{\textbf{.797}} & \textcolor{tabred}{\textbf{32.51}} &  \textcolor{tabred}{\textbf{.916}} \\
     \bottomrule
    \end{tabularx}
    \vspace{-4mm}
\end{table*}

==> tables/supp_capacity.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \setlength\tabcolsep{1.8pt}
    \setlength{\extrarowheight}{0.5pt}
    \caption{\textit{Network Capacity and Complexity Analysis on Deraining.} Comparison of PSNR, model parameters, and FLOPs, highlighting the balance between network capacity and computational efficiency. FLOPs are computed for $224\times224$ input images using an NVIDIA Tesla A100 (40G) GPU.}
    \vspace{-3mm}
    \label{tab:supp_capacity}
    \begin{tabularx}{\columnwidth}{X*{5}{c}}
    % \begin{tabularx}{\textwidth}{X*{3}{c}}
        \toprule
        Method  &Blocks &PSNR (dB, $\uparrow$) &Params. ($\downarrow$) & FLOPs ($\downarrow$) \\
        \midrule
        PromptIR~\cite{potlapalli2023promptir}(Base) & [4,6,6,8] &37.04 & 35.6M & 132G \\
        Base (No Prompt)& [4,6,6,8] & 36.74 & 32.2M & 117G \\
        Base (Fix-Prompt) & [4,6,6,8] & 36.85 & - & -  \\
        \midrule
        Base (No Prompt) & [3,5,5,7] & 36.84 & 29.1M & 101G \\
        Base (No Prompt) & [2,4,4,6] & 36.76 & 26.0M & 85G \\
        Base (No Prompt) & [1,3,3,5] & 36.63 & 22.9M & 68G \\
        \midrule
        \ourmethod(\textit{ours}) & [3,5,5,7] &\textcolor{tabred}{\textbf{37.79}} & \textcolor{tabred}{\textbf{6.3M}} & \textcolor{tabred}{\textbf{19G}} \\ 
        \bottomrule
    \end{tabularx}
    \vspace{-2.4em}
\end{table}


==> tables/supp_inference.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \setlength\tabcolsep{2.5pt}
    \caption{Full \textbf{inference time} comparison under the 3-degradation all-in-one IR setting. The lower the better.}
    \vspace{-2mm}
    \label{tab:inferencetime}
    \setlength{\extrarowheight}{2pt}
    \setlength\tabcolsep{4pt}
    \scalebox{1}{
    \begin{tabularx}{\columnwidth}{X*{4}{c}}
    % \begin{tabularx}{\textwidth}{X*{3}{c}}
        \toprule
        Task  & Num. Samples & PromptIR~\cite{potlapalli2023promptir} & \ourmethod (Ours)  \\
        \midrule
        Denoising ($\sigma=15$)& 68 & 41s & 30s \\ 
        Denoising ($\sigma=25$)& 68 & 41s & 30s \\ 
        Denoising ($\sigma=50$)& 68 & 42s & 30s \\ 
        \midrule
        Deraining & 100 & 60s & 43s \\ 
        \midrule
        Dehazing & 500 & 416s & 274s\\
        \midrule
        Frames Per Second & - & 1.34 & 1.97\\
        \bottomrule        
    \end{tabularx}
    }
    \vspace{0mm}
\end{table}

==> tables/supp_mixdeg.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \setlength\tabcolsep{1pt} 
    \caption{\textbf{Mixed degradation} result with the CDD-11~\cite{guo2024onerestore} dataset.}
    \vspace{-2mm}
    \label{tab:supp_mix}
    \begin{tabularx}{\columnwidth}{>{\raggedright\arraybackslash}m{3.1cm}c@{\hskip 10pt}c@{\hskip 20pt}c@{\hskip 8pt}c}
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{low-light+haze+rain} & \multicolumn{2}{c}{low-light+haze+snow} \\
        \cmidrule(r){2-3} \cmidrule(r){4-5} % 短线范围优化
        & PSNR & SSIM & PSNR & SSIM \\
        \midrule
        AirNet~\cite{li2022airnet} & 21.80 & .708 & 22.23 & .725 \\
        TransWeather~\cite{valanarasu2022transweather} & 21.55 & .678 & 21.01 & .655 \\
        % WeatherDiff & 21.23 & .716 & 21.03 & .698 \\
        PromptIR~\cite{potlapalli2023promptir} & 23.51 & .752 & 23.33 & .747 \\
        \ourmethod (Ours) & \textcolor{tabred}{\textbf{24.54}} & \textcolor{tabred}{\textbf{.783}} & \textcolor{tabred}{\textbf{24.67}} & \textcolor{tabred}{\textbf{.790}} \\
        % OneRestore & 25.18 & .795 & 25.28 & .797 \\
        \bottomrule
    \end{tabularx}
    \vspace{-3mm}
\end{table}

==> tables/supp_unseen.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \setlength\tabcolsep{2.0pt}
    \caption{Unseen \textbf{Desnowing} comparison with the CSD~\cite{chen2021all} dataset.}
    \vspace{-2mm}
    \label{tab:supp_unseen}
    \setlength{\extrarowheight}{2pt}
    \setlength\tabcolsep{4pt}
    \scalebox{1}{
    \begin{tabularx}{\columnwidth}{X*{4}{c}}
    % \begin{tabularx}{\textwidth}{X*{3}{c}}
        \toprule
        Method  & AirNet~\cite{li2022airnet} & PromptIR~\cite{potlapalli2023promptir} & \ourmethod (Ours)  \\
        \midrule
        PSNR & 19.32 & 20.47 & \textcolor{tabred}{\textbf{21.54}} \\ 
        SSIM & .733 & .764 & \textcolor{tabred}{\textbf{.781}} \\ 
        \bottomrule        
    \end{tabularx}
    }
    \vspace{-1mm}
\end{table}
